NICE: Improving Panoptic Narrative Detection and Segmentation with Cascading Collaborative Learning

Panoptic Narrative Detection (PND) and Segmentation (PNS) are two challenging tasks that involve identifying and locating multiple targets in an image according to a long narrative description. In this paper, we propose a unified and effective framework called NICE that can jointly learn these two panoptic narrative recognition tasks. Existing visual grounding tasks use a two-branch paradigm, but applying this directly to PND and PNS can result in prediction conflict due to their intrinsic many-to-many alignment property. To address this, we introduce two cascading modules based on the barycenter of the mask, which are Coordinate Guided Aggregation (CGA) and Barycenter Driven Localization (BDL), responsible for segmentation and detection, respectively. By linking PNS and PND in series with the barycenter of segmentation as the anchor, our approach naturally aligns the two tasks and allows them to complement each other for improved performance. Specifically, CGA provides the barycenter as a reference for detection, reducing BDL's reliance on a large number of candidate boxes. BDL leverages its excellent properties to distinguish different instances, which improves the performance of CGA for segmentation. Extensive experiments demonstrate that NICE surpasses all existing methods by a large margin, achieving 4.1% for PND and 2.9% for PNS over the state-of-the-art. These results validate the effectiveness of our proposed collaborative learning strategy. The project of this work is made publicly available at https://github.com/Mr-Neko/NICE.

==> tables/ie.tex <==
\begin{table}[t]
\centering
\resizebox{0.96\linewidth}{!}{
\begin{tabular}{l|ccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{3}{|c}{IE $\downarrow$}\\

\cline{2-4}
 & Overall & wrong mask & wrong box \\

\hline

MCN & 20.3\% &  9.6\% & 10.7\% \\


% ours 18.3  0.063 0.120
% mask 30.5  0.064  0.241
% mcn  20.     0.097  0.107
% two 27.2 9.8 17.4
\hline

NICE$^{\dagger}$ & 27.2\% & 9.8\% & 17.4\% \\
NICE$^{*}$ & 30.5\% & 6.4\% & 24.1\%\\
NICE & 18.3\% & 6.3\% & 12.0\% \\
 \bottomrule
\end{tabular}
}
\caption{Comparison of the models in IE, which is used to evaluate the severity of the prediction conflict.}
\label{ie}

\end{table}

==> tables/table1.tex <==
\begin{table*}[t!]
\centering
\resizebox{0.96\linewidth}{!}{
\begin{tabular}{l|cccccc|cccccc|c|c|c}
\toprule
\multirow{2}{*}{Method} & \multicolumn{6}{|c|}{Segmentation Average Recall} & \multicolumn{6}{|c|}{Detection Average Recall} & \multirow{2}{*}{IE $\downarrow$} & \multirow{2}{*}{Gflops} & \multirow{2}{*}{Params} \\

\cline{2-13}
 & All & Thing & Stuff & Single & Plural & Time & All & Thing & Stuff & Single & Plural & Time & & & \\

\hline
PNG~\cite{gonzalez2021panoptic} & 55.4 & 56.2 & 54.3 & 56.2 & 48.8 & 107ms & -& -& -& -& - &- &- & \textbf{62.5} & 100.1 M \\
EPNG~\cite{wang2023towards} & 58.0 & 54.8 & 62.4 & 58.6 & 52.1 & \textbf{11ms} & -& -& -& -& - &- &- & 259.5 & 24.2 M \\
PPMN~\cite{ding2022ppmn} & 59.4 & 57.2 & 62.5 & 60.0 & 50.4 & 63.5ms & -& -& -& -& - &- &- & 241.1 & 10 M\\
RefTR~\cite{li2021referring}  & - & - & - & - & - & - & 53.6 & 47.2 & 62.4 & 54.0 & 50.2 & 82.1ms & - & 808.1 & 12.3 M\\
MCN~\cite{luo2020multi} & 54.2 & 48.6 & 61.4 & 56.6 & 38.8 & 146.3ms & 49.9 & 49.8 & 50.0 & 50.7 & 44.7& 146.3ms & 20.3\% & 342.8 & 14.5 M\\


% ours 18.3  0.063 0.120
% mask 30.5  0.064  0.241
% mcn  20.     0.097  0.107
% two 27.2 9.8 17.4
\hline

NICE$^{\dagger}$ & 58.6 & 56.0 & 62.2 & 59.5 & 50.1 & 49.2ms & 45.4 & 37.8 & 55.8 & 45.6 & 43.7 & \textbf{49.2ms}& 27.2\% & 164.0 & 8.6 M\\
NICE$^{*}$ & 60.8 & 58.7 & 63.8 & 61.7 & 52.8 & 49.2ms & 47.5 & 39.3 & 58.8 & 47.8 & 44.7 & 53.6ms & 30.5\% & 164.0 & \textbf{8.6 M}\\
NICE & \textbf{62.3} & \textbf{60.2} & \textbf{65.3} & \textbf{63.1} & \textbf{55.2} & 49.2ms & \textbf{57.7} & \textbf{54.1} & \textbf{62.7} & \textbf{58.7} & \textbf{49.2} & 56.9 ms & \textbf{18.3\%} & 285.2 & 10.9 M\\

 \bottomrule
\end{tabular}
}
\caption{Comparison of the NICE and the state-of-the-art methods. MCN is a mluti-task learning method with a two-branch structure. NICE$^{\dagger}$ is the variant using the two-branch design, just like MCN. NICE$^{*}$ directly finds the smallest rectangular box that can enclose the mask as the detection box.}
\label{table1}
\vspace{-0.3em}
\end{table*}

==> tables/table2.tex <==
\begin{table}[t]
\centering
\resizebox{1.00\linewidth}{!}{
\begin{tabular}{l|ccccc|ccccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{5}{|c|}{Segmentation Average Recall} & \multicolumn{5}{|c}{Detection Average Recall}\\

\cline{2-11}
 & All & Thing & Stuff & Single & Plural & All & Thing & Stuff & Single & Plural\\

\hline
OnlyBox & - & - & - & - & - & 43.2 & 37.4 & 51.2 & 43.3 & 42.2\\
OnlyMask & 58.1 & 54.6 & 63.0 & 59.3 & 47.9 & -& -& -& -& -\\
NICE &\textbf{62.3} & \textbf{60.2} & \textbf{65.3} & \textbf{63.1} & \textbf{55.2} & \textbf{57.7} & \textbf{54.1} & \textbf{62.7} & \textbf{58.7} & \textbf{49.2}\\

 \bottomrule
\end{tabular}}
%}
\caption{Ablation study of single and multi-task learning. OnlyBox and OnlyMask are single-task learning.}
\label{table2}
\vspace{-0.5em}
\end{table}

==> tables/table3.tex <==
\begin{table}[t!]
\centering
\resizebox{1.00\linewidth}{!}{
\begin{tabular}{c|c|ccccc|ccccc}
\toprule
\multicolumn{2}{c|}{Method} & \multicolumn{5}{|c|}{Segmentation Average Recall} & \multicolumn{5}{|c}{Detection Average Recall}\\

\hline
 CGA & BDL & All & Thing & Stuff & Single & Plural & All & Thing & Stuff & Single & Plural\\

\hline
\ding{55} & \ding{55} & 58.6 & 56.0 & 62.2 & 59.5 & 50.1 & 45.4 & 37.8 & 55.8 & 45.6 & 43.7 \\
\ding{51} & \ding{55} & 60.4 & 57.7 & 64.0 & 61.2 & 52.6 & 45.9 & 33 & \textbf{63.9} & 46.3 & 42.9\\
\ding{51} & \ding{51} & \textbf{62.3} & \textbf{60.2} & \textbf{65.3} & \textbf{63.1} & \textbf{55.2} & \textbf{57.7} & \textbf{54.1} & 62.7 & \textbf{58.7} & \textbf{49.2}\\

 \bottomrule
\end{tabular}}
%}
\caption{Ablation study of CGA and BDL.}
\label{table3}
%\vspace{-1em}
\end{table}

==> tables/table4.tex <==
\begin{table}[t!]
\centering
\resizebox{1.00\linewidth}{!}{
\begin{tabular}{l|ccccc|ccccc}
\toprule
\multirow{2}{*}{Barycenter} & \multicolumn{5}{|c|}{Segmentation Average Recall} & \multicolumn{5}{|c}{Detection Average Recall}\\

\cline{2-11}
 & All & Thing & Stuff & Single & Plural & All & Thing & Stuff & Single & Plural\\

\hline
Top1 & 59.6 & 56.5 & 63.8 & 60.4 & 51.9 & 30.4 & 22.9 & 40.9 & 30.4 & 30.3\\
Top50 & 61.1 & 58.7 & 64.5 & 62 & 52.6 & 41.1 & 37.2 & 46.6 & 41.9 & 33.9\\
Top100 & 59.7 & 57.1 & 63.3 & 60.7 & 50.6 & 35.1 & 31.2 & 40.5 & 35.6 & 30.0\\
Average &\textbf{62.3} & \textbf{60.2} & \textbf{65.3} & \textbf{63.1} & \textbf{55.2} & \textbf{57.7} & \textbf{54.1} & \textbf{62.7} & \textbf{58.7} & \textbf{49.2}\\

 \bottomrule
\end{tabular}}
%}
\caption{Ablation study of the settings of barycenters.}
\label{table4}
\end{table}

==> tables/table5.tex <==
\begin{table*}[t!]
\centering
\resizebox{!}{!}{
\begin{tabular}{l|ccccc|ccccc}
\toprule
\multirow{2}{*}{Scale} & \multicolumn{5}{|c|}{Segmentation Average Recall} & \multicolumn{5}{|c}{Detection Average Recall}\\

\cline{2-11}
 & All & Thing & Stuff & Single & Plural & All & Thing & Stuff & Single & Plural\\

\hline
Mluti-scale & 60.5 & 58.1 & 63.8 & 61.4 & 52.3 & \textbf{58.7} & 54.0 & \textbf{65.2} & \textbf{59.7} & \textbf{49.7}\\
Fusion &\textbf{62.3} & \textbf{60.2} & \textbf{65.3} & \textbf{63.1} & \textbf{55.2} & 57.7 & \textbf{54.1} & 62.7 & 58.7 & 49.2\\

 \bottomrule
\end{tabular}}
%}
\caption{Ablation study of scales in BDL.}
\label{table5}
\vspace{-0.5em}
\end{table*}

==> tables/table6.tex <==
\begin{table}[]
\centering
\resizebox{1.00\linewidth}{!}{
\begin{tabular}{l|ccccc|ccccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{5}{|c|}{Segmentation Average Recall} & \multicolumn{5}{|c}{Detection Average Recall}\\

\cline{2-11}
 & All & Thing & Stuff & Single & Plural & All & Thing & Stuff & Single & Plural\\

\hline
NICE &\textbf{62.3} & \textbf{60.2} & \textbf{65.3} & \textbf{63.1} & \textbf{55.2} & \textbf{57.7} & \textbf{54.1} & \textbf{62.7} & \textbf{58.7} & \textbf{49.2}\\
w/o stuff & 59.0 & 56.1 & 63.2 & 59.7 & 53.2 & 48.9 & 48.9 & -& 46.4& 46.7\\

 \bottomrule
\end{tabular}}
%}
\caption{Ablation study of with and without stuff. }
\label{tab: stuff}
\end{table}

==> tables/table_zs_b.tex <==
% tabel5
\begin{table*}[t]
\centering

\begin{tabular}{c|c|c|ccccc}
\toprule
 \multicolumn{2}{c|}{Dataset} & Type & AP@0.1 & AP@0.2 & AP@0.3 & AP@0.4 & AP@0.5\\
 \hline
 \multirow{4}{*}{RefCOCO} & \multirow{2}{*}{testA} & randn & 66.7 & 34.1 & 17.4 & 9.0 & 4.2 \\
 \cline{3-3}
  & & zero-shot & 67.4 & 57.4 & 48.5 & 39.3 & 32.3\\
  \cline{2-8}
  & \multirow{2}{*}{testB} & randn & 67.9 & 33.8 & 17.6 & 8.8 & 5.0 \\
 \cline{3-3}
  & & zero-shot & 77.6 & 61.2 & 47.6 & 35.8 & 27.4\\
  
  \hline
 \multirow{4}{*}{RefCOCO+} & \multirow{2}{*}{testA} & randn & 63.8 & 32.1 & 16.4 & 8.4 & 3.8 \\
 \cline{3-3}
  & & zero-shot & 54.8 & 43.0 & 33.2 & 24.8 & 18.6\\
  \cline{2-8}
  & \multirow{2}{*}{testB} & randn & 67.4 & 34.1 & 17.5 & 8.9 & 5.1 \\
 \cline{3-3}
  & & zero-shot & 68.4 & 50.8 & 37.8 & 26.1 & 18.5\\
  
\hline
 \multirow{2}{*}{RefCOCOg} & \multirow{2}{*}{test} & randn & 67.6 & 36.4 & 21.2 & 12.8 & 7.4 \\
 \cline{3-3}
  & & zero-shot & 80.0 & 63.4 & 47.4 & 34.0 & 23.5\\

 \bottomrule
\end{tabular}
%}
\caption{Zero-shot results of Nice on REC. We cacluate the precious when the threshold of IoU is from 0.1 to 0.5.}
\label{tablezb}
%\vspace{-0.4cm}
\end{table*}

==> tables/table_zs_s.tex <==
% tabel5
\begin{table*}[t]
\centering
\begin{tabular}{c|c|c|ccccc}
\toprule
 \multicolumn{2}{c|}{Dataset} & Type & AP@0.1 & AP@0.2 & AP@0.3 & AP@0.4 & AP@0.5\\
 \hline
 \multirow{4}{*}{RefCOCO} & \multirow{2}{*}{testA} & randn & 36.2 & 10.4 & 3.3 & 1.1 & 0.2 \\
 \cline{3-3}
  & & zero-shot & 51.0 & 47.4 & 43.4 & 39.3 & 34.8\\
  \cline{2-8}
  & \multirow{2}{*}{testB} & randn & 40.1 & 13.2 & 5.0 & 2.3 & 0.6 \\
 \cline{3-3}
  & & zero-shot & 60.6 & 53.0 & 45.9 & 37.8 & 30.0\\
  
  \hline
 \multirow{4}{*}{RefCOCO+} & \multirow{2}{*}{testA} & randn & 34.1 & 9.7 & 3.0 & 1.1 & 0.1 \\
 \cline{3-3}
  & & zero-shot & 34.1 & 29.9 & 26.8 & 23.4 & 19.6\\
  \cline{2-8}
  & \multirow{2}{*}{testB} & randn & 40.3 & 12.9 & 5.1  & 2.5 & 0.6 \\
 \cline{3-3}
  & & zero-shot & 44.0 & 37.0 & 30.9 & 24.5 & 18.8\\
  
\hline
 \multirow{2}{*}{RefCOCOg} & \multirow{2}{*}{test} & randn & 39.0 & 14.9 & 5.8 & 2.3 & 1.0 \\
 \cline{3-3}
  & & zero-shot & 46.6 & 41.2 & 36.6 & 31.4 & 26.2\\

 \bottomrule
\end{tabular}
%}
\caption{Zero-shot results of Nice on RES. We cacluate the precious when the threshold of IoU is from 0.1 to 0.5.}
\label{tablezs}
%\vspace{-0.4cm}
\end{table*}
